Can ChatGPT Support Developers? An Empirical Evaluation of Large Language Models for Code Generation

Large language models (LLMs) have demonstrated notable proficiency in code generation, with numerous prior studies showing their promising capabilities in various development scenarios. However, these studies mainly provide evaluations in research settings, which leaves a significant gap in understanding how effectively LLMs can support developers in real-world. To address this, we conducted an empirical analysis of conversations in DevGPT, a dataset collected from developers' conversations with ChatGPT (captured with the Share Link feature on platforms such as GitHub). Our empirical findings indicate that the current practice of using LLM-generated code is typically limited to either demonstrating high-level concepts or providing examples in documentation, rather than to be used as production-ready code. These findings indicate that there is much future work needed to improve LLMs in code generation before they can be integral parts of modern software development.

==> code/RQ2_modified_example.tex <==
%New colors defined below
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

%Code listing style named "mystyle"
\lstdefinestyle{mystyle}{
  backgroundcolor=\color{backcolour}, commentstyle=\color{codegreen},
  keywordstyle=\color{magenta},
  numberstyle=\tiny\color{codegray},
  stringstyle=\color{codepurple},
  basicstyle=\ttfamily\footnotesize,
  breakatwhitespace=false,         
  breaklines=true,                 
  captionpos=b,                    
  keepspaces=true,                 
  numbers=left,                    
  numbersep=5pt,                  
  showspaces=false,                
  showstringspaces=false,
  showtabs=false,                  
  tabsize=2
}
\begin{figure}
%"mystyle" code listing set
\lstset{style=mystyle}
\begin{lstlisting}[language=Python]
def get_more_movies(request):
    page_number = 1
    try:
        page_number = int(request.GET.get("page", 1)
    except ValueError:
        #Handle the case when the "page" parameter is not a valid integer
        #You can choose to display an error message or set a default value

    movies_per_page = NUMBER_MOVIES_PER_PAGE
    ...
\end{lstlisting}
\vspace{-5pt}
\caption{Modified generated code used in django's paginator}
\label{fig:modified_code}
\vspace{-5pt}
\end{figure}

==> figs/RQ11_conversation_example.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figs/Conversation_example.png}
  \caption{An example of redundant conversation rounds
  }
  \label{fig:Conversation_example}
\end{figure}


==> figs/RQ11_num_avg_round.tex <==
% \begin{figure}
%    \includegraphics[width=\linewidth]{figs/Code_Generation_Distributions.png}
%    \caption{Distribution of conversation volume associated with code generation.}
%    \label{fig:Code_Generation_Distributions}
%  \end{figure}
\vspace{-5pt}
\begin{figure}
  \vspace{-5pt}
  \includegraphics[width=0.9\linewidth]{figs/Conversation_Round_Distributions_modified.png}
  \vspace{-5pt}
  \caption{The number of prompt-response rounds for 
  %depicted for 
  each GitHub category
  %, with the x-axis representing the rounds involved in each conversation, and the y-axis denoting the five distinct categories on GitHub.
  }
  \label{fig:Conversation_Round_Distributions}
  \vspace{-5pt}
\end{figure}

==> figs/RQ2_document_example.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figs/Document_example.png}
  \caption{An example of code generation for documents.
  %(How the generated code is used)
  }
  \label{fig:Document_example}
\end{figure}

==> figs/RQ2_modified_example.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figs/Modified_example.png}
  \caption{An example of developers modifying code before including it in the source code.
  %(How the generated code is used)
  }
  \label{fig:Modified_example}
\end{figure}

==> figs/RQ2_not_used_example.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figs/Not-used-example.png}
  \caption{An example of Not Used reasons.
  %(How the generated code is used)
  }
  \label{fig:Not_used example}
\end{figure}

==> figs/pickJS.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figs/pickJS.png}
  \caption{An example for Exact Matches
  %(How the generated code is used)
  }
  \label{fig:EM}
\end{figure}
